Quantization of charged fields in the presence of intense electromagnetic fields

This thesis applies techniques from quantum field theory in curved spacetimes to study particle creation in external fields, focusing on the Schwinger effect (i.e., the production of particle-antiparticle pairs by intense electric fields). Although experimental verification remains out of reach, theoretical analysis advances our understanding of this phenomenon and its broader implications. The work develops the theoretical framework for quantizing charged fields in nontrivial backgrounds, addressing the ambiguities in defining the quantum vacuum and extending the concept of states of low energy from cosmology to the Schwinger setting. It examines how different quantizations allow for unitary time evolution, and generalizes the quantum Vlasov equation to encompass a wider range of schemes. An operational perspective reveals that quantum ambiguities have genuine physical meaning, being linked to different modes of interaction and measurement. The study also analyzes dynamical transitions between static regimes and their impact on observables, with applications to analog cosmological expansion in Bose-Einstein condensates and the Schwinger effect itself. In the context of black holes, the thesis shows that the Schwinger effect prevents the formation of black holes from light under current conditions and investigates fermionic charge superradiance, demonstrating how quantum effects lead to black-hole discharge (a process without classical analogue). Overall, the thesis underscores the fundamental role of external electromagnetic and gravitational fields in defining particles and vacua, revealing the limits of flat-spacetime intuition and identifying purely quantum phenomena with implications for black-hole physics. It contributes to bridging the conceptual gap between general relativity and quantum field theory and offers new tools toward a consistent quantum description of spacetime.

==> Matter/06-Appendices.tex <==
\ifthenelse{\equal{\LanguageOption}{portuguese}}{
    \addtocontents{toc}{\protect\contentsline{chapter}{Apêndices}{}{}}
}{
    \addtocontents{toc}{\protect\contentsline{chapter}{Appendices}{}{}}
}

\blankpage
\begin{center}
    %\minionfont
    \thispagestyle{empty}
        
    \vspace*{\fill}
    \ifthenelse{\equal{\LanguageOption}{portuguese}}{%
        {\LARGE\fontsize{26}{26}\selectfont\textcolor{darkred}{Apêndices}\par}
    }{%
        {\LARGE\fontsize{26}{26}\selectfont\textcolor{darkred}{Appendices}\par}
    }
    \vspace*{\fill}
\end{center}
\blankpage

==> Matter/07-Annexes.tex <==
\ifthenelse{\equal{\LanguageOption}{portuguese}}{
    \addtocontents{toc}{\protect\contentsline{chapter}{Anexos}{}{}}
}{
    \addtocontents{toc}{\protect\contentsline{chapter}{Annexes}{}{}}
}

\setcounter{chapter}{11} % To start at the "L" chapter.
\blankpage
\begin{center}
    %\minionfont
    \thispagestyle{empty}
        
    \vspace*{\fill}
    \ifthenelse{\equal{\LanguageOption}{portuguese}}{%
        {\LARGE\fontsize{26}{26}\selectfont\textcolor{darkred}{Anexos}\par}
    }{%
        {\LARGE\fontsize{26}{26}\selectfont\textcolor{darkred}{Annexes}\par}
    }
    \vspace*{\fill}
\end{center}
\blankpage
